Dynamic Entity Representations in Neural Language Models

Understanding a long document requires tracking how entities are introduced and evolve over time. We present a new type of language model, EntityNLM, that can explicitly model entities, dynamically update their representations, and contextually generate their mentions. Our model is generative and flexible; it can model an arbitrary number of entities in context while generating each entity mention at an arbitrary length. In addition, it can be used for several different tasks such as language modeling, coreference resolution, and entity prediction. Experimental results with all these tasks demonstrate that our model consistently outperforms strong baselines and prior work.

==> figures/entity-gen.tex <==

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../language"
%%% End:

\tikzstyle{comp}=[rectangle,
thick,
minimum width=2.0cm,
draw=black!80]

\begin{tikzpicture}[>=latex,text height=1.5ex,text depth=0.25ex]
  \matrix[row sep=1.0cm,column sep=1.6cm] {
    & \node (R) [comp] {Entity Type $R$}; & \\
    & \node (E) [comp] {Entity $E$}; & \\
    & \node (M) [comp] {Mention $X$ with length $L$}; & \\
  };
  \path[->]
  (R) edge[thick] (E)
  (E) edge[thick] (M);
\end{tikzpicture}


==> figures/model.tex <==

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../language"
%%% End:

\tikzstyle{randomvar}=[circle,
thick,
minimum size=1.2cm,
draw=blue!80,
fill=blue!20]

\tikzstyle{hidden}=[circle,
thick,
minimum size=1.2cm,
draw=black!80]

\begin{tikzpicture}[>=latex,text height=1.5ex,text depth=0.25ex]
  \matrix[row sep=1.0cm,column sep=1.6cm] {
    &
    \node (t_t) [randomvar] {$R_t$}; &
    & 
    \node (t_tplus1) [randomvar] {$R_{t+1}$}; &
    \\
    % Entity 
    & 
    \node (e_t) [randomvar] {$E_t$}; & 
    & 
    \node (e_tplus1) [randomvar] {$E_{t+1}$}; &
    \\
    % Entity length
    & 
    \node (l_t) [randomvar] {$L_t$}; & 
    & 
    \node (l_tplus1) [randomvar] {$L_{t+1}$}; &
    \\
    % Hidden layer
    \node (h_tminus1) [hidden] {$\vec{h}_{t-1}$}; &
    &
    \node (h_t) [hidden] {$\vec{h}_{t}$}; &
    &
    \node (h_tplus1) [hidden] {$\vec{h}_{t+1}$}; \\
    % Word sequence
    \node (x_tminus1) [randomvar] {$X_{t-1}$};  & 
    &
    \node (x_t) [randomvar] {$X_{t}$};   &
    &
    \node (x_tplus1) [randomvar] {$X_{t+1}$}; \\
  };
  \path[->]
  % word -> hidden
  (x_tminus1) edge[thick] (h_tminus1)
  (x_t) edge[thick] (h_t)
  (x_tplus1) edge[thick] (h_tplus1)
  % type -> type
  (t_t) edge[dashed] (t_tplus1)
  % type -> entity
  (t_t) edge[dashed] (e_t)
  (t_tplus1) edge[dashed] (e_tplus1)
  % type -> word
  % (t_t) edge[dashed] (x_t)
  % (t_tplus1) edge[dashed] (x_tplus1)
  % entity -> entity
  (e_t) edge[dashed] (e_tplus1)
  % entity -> length
  (e_t) edge[dashed] (l_t)
  (e_t) edge[dashed] (l_tplus1)
  (e_tplus1) edge[dashed] (l_tplus1)
  % entity -> word
  (e_t) edge[dashed] (x_t)
  (e_tplus1) edge[dashed] (x_tplus1)
  % length -> length
  (l_t) edge[dashed] (l_tplus1)
  % length -> type
  (l_t) edge[dashed] (t_tplus1)
  % length -> entity
  (l_t) edge[dashed] (e_tplus1)
  % length -> word
  (l_t) edge[dashed] (x_t)
  (l_tplus1) edge[dashed] (x_tplus1)
  % hidden -> hidden
  (h_tminus1) edge[thick] (h_t)
  (h_t) edge[thick] (h_tplus1)
  % hidden -> type
  (h_tminus1) edge[dashed] (t_t)
  (h_t) edge[dashed] (t_tplus1)
  % hidden -> entity
  (h_tminus1) edge[dashed] (e_t)
  (h_t) edge[dashed] (e_tplus1)
  % hidden -> length
  (h_tminus1) edge[dashed] (l_t)
  (h_t) edge[dashed] (l_tplus1)
  % hidden -> word
  (h_tminus1) edge[dashed] (x_t)
  (h_t) edge[dashed] (x_tplus1)
  ;
\end{tikzpicture}


==> idea.tex <==
%!TEX root = main.tex

\section{A Generative Model for Entities}
\label{sec:idea}

Inspired by \citet{haghighi2010coreference}, we propose a hierarchical procedure for entity generation. 
As illustrated in \autoref{fig:entity-gen}, the whole procedure take three steps to generate a entity mention. 
First, it predicts the entity type given the contextual information (and some other discourse information, we will explained later). 
For a given entity type, it further predicts which entity should be referred. 
Then, the last step is to realize a specific mention that belongs to the predicted entity.
\chenhao{Do we actually use entity types in our final model? This seems different.}

\begin{figure}
  \centering
  \input{figures/entity-gen}
  \caption{The abstraction of entity generation.}
  \label{fig:entity-gen}
\end{figure}

The way of defining entity types could be any categorization on entities. 
A reasonable categorization would allow the entity type based information to be shared across different texts/documents. 
For example, in \citet{haghighi2010coreference}, the entity types include \rela{Org}, \rela{Person}, etc. 
In addition, we expect to use a unified generative procedure for entity mention words and non-mention words and each time step will only generate a single token.
Therefore, the model needs a dedicated component to handle different lengths of mentions for the same entity, e.g., \enttwo{coffee shop} and \enttwo{it} in \autoref{fig:example}. 
For that, we introduce a semi-Markov framework on the top of RNNLM. 


==> notations.tex <==
\section{Notations}

\begin{itemize}
\item $R_t$: random variable; the entity type at time $t$, where the sample space is $T_t\in\{\text{\sc None}, \text{\sc Org}, \text{\sc Person}, \dots\}$
\item $E_t$: random variable; the entity index at time $t$, where the sample space is $E_t\in\{0,1,\dots,K\}$ and $K$ is the number of the entity clusters, where $E_t=0$ means a new entity
\item $L_t$: random variable; the segment length, each segment could be a entity mention ($L_t\geq 1$) and just a normal word ($L_t = 1$)
\item $X_t$: random variable; the word index at time $t$, where each of $X_t=x_t$ is a one-hot vector
\item $\vec{h}_t$: vector; the RNN hidden state at time $t$
\item $\mat{W}_{\cdot}$: matrix; parameter
\item $\vec{v}_{\cdot}$: vector; (entity or word) embedding
\end{itemize}

==> sampling.tex <==
\section{Approximate Sampling in cort}
\label{app:sampling}
